PolyGET: Accelerating Polymer Simulations by Accurate and Generalizable Forcefield with Equivariant Transformer

Polymer simulation with both accuracy and efficiency is a challenging task. Machine learning (ML) forcefields have been developed to achieve both the accuracy of ab initio methods and the efficiency of empirical force fields. However, existing ML force fields are usually limited to single-molecule settings, and their simulations are not robust enough. In this paper, we present PolyGET, a new framework for Polymer Forcefields with Generalizable Equivariant Transformers. PolyGET is designed to capture complex quantum interactions between atoms and generalize across various polymer families, using a deep learning model called Equivariant Transformers. We propose a new training paradigm that focuses exclusively on optimizing forces, which is different from existing methods that jointly optimize forces and energy. This simple force-centric objective function avoids competing objectives between energy and forces, thereby allowing for learning a unified forcefield ML model over different polymer families. We evaluated PolyGET on a large-scale dataset of 24 distinct polymer types and demonstrated state-of-the-art performance in force accuracy and robust MD simulations. Furthermore, PolyGET can simulate large polymers with high fidelity to the reference ab initio DFT method while being able to generalize to unseen polymers.

==> comp_gen_table.tex <==
\begin{table}[]
\begin{tabular}{llllll}
Pretrain Size & Molecule & Loop & Energy Correlation & Forces (eV/A) & Forces Correlation \\
  1            & 49       & 5    &       0.808             &       0.033        &      0.974              \\
    1          &   49       &   6   &      0.516              &           0.030    &     0.972               \\
     1         &    51      &  5 &  0.926   &        0.019            &               0.982 \\           
          1         &    51      &  6 &  0.826   &        0.035            &               0.970 \\  
          
\end{tabular}
\label{tab:comp_gen}
\end{table}

==> demo.tex <==
\section{Na\"ive Training Across Molecules}



==> exp_monomer.tex <==

\hide{
\subsection{Multi-molecule Forces Prediction Performance}
\label{sec:exp:multimolecule}

% In Section~\ref{sec:exp:sim_robust} it will be further analyzed that the multi-molecule training paradigm is the key to increased accuracy and robustness in simulation.
In this section, we analyze the benefit brought from multi-molecule training. 
We show that introducing the multi-molecule training paradigm greatly increases the model's capacity to produce accurate forces and extrapolate to unseen and larger polymers.
%The training set consists of the DFT trajectories of the monomers of all 24 polymers. For each monomer, 9 trajectories are taken for training and validation. The last trajectory is used for testing the model performance, where the model-predicted forces are compared with DFT forces on the DFT trajectories.

Figure~\ref{fig:multimodel} compares the DFT accuracy. Specifically, Figure~\ref{fig:multimodel_mae} shows the Mean Squared Error for all models, which is averaged across four types of polymer. Meanwhile, Figures~\ref{fig:multimodel}(b)-(e) present scatter plots of DFT forces versus predicted forces, illustrating the correlation between predicted and DFT forces. These figures demonstrate that our model, \ours, consistently produces accurate forces for all polymers tested. On average, our model achieves a MAE of 0.0073 on forces compared to DFT forces, which is five times lower than the best baseline model, TorchMDNet. Furthermore, the cosine distance of our model is close to zero, further indicating its high accuracy.

% \paragraph*{Particularly, \ours~ benefits significantly from the diversity of molecules present in the training set.} To evaluate the performance of jointly and separately trained models, we conducted experiments on five different monomers of five polymer types: \texttt{CK4}, \texttt{CK5}, \texttt{LAC8}, \texttt{OTH5}, and \texttt{OTH8}. The comparison of NequIP, TorchMDNet, and \ours~ is shown in Figure~\ref{fig:static:single_multi}, where the boxplot visualizes the distribution of model MAE on forces across all evaluated polymers. Our results indicate that for NequIP and TorchMDNet, introducing diverse polymer types in the training data does not improve, and could even worsen, the model performance. However, \ours~ diverse training set of polymer types enables it to achieve a substantial improvement in performance, reducing the average MAE from 0.032 to 0.005 eV/\AA across the five polymers.

We have also conducted experiments to show \ours
benefits significantly from the diversity of training molecules.
Our experiments evaluated the performance of jointly and separately trained models using five different monomers from five polymer types: \texttt{CK4}, \texttt{CK5}, \texttt{LAC8}, \texttt{OTH5}, and \texttt{OTH8}. Figure~\ref{fig:static:single_multi} compares NequIP, TorchMDNet, and \ours~ using a boxplot to visualize the distribution of model MAE on forces across all evaluated polymers. Our results reveal that introducing diverse polymer types to the training data does not improve the model performance for NequIP and TorchMDNet, and could even worsen it. However, \ours~ benefits significantly from the diversity of molecules present in the training set, allowing it to achieve a substantial improvement in performance. Specifically, the average MAE across the five polymers was reduced from 0.032 to 0.005 eV/\AA~ when using \ours~ with a diverse training set of polymer types.

We have also found that \ours~ extrapolates well to polymers of different sizes and unseen polymer types.
In Figure~\ref{fig:static:seen_unseen} we visualize \ours's performance on unseen polymers. Specifically, ``unseen'' polymers are 6-loop polymer data that are not observed by the model during the training stage. For each polymer type, the 6-loop has similar structures with the lesser loop polymers but is larger in polymer size. Without further training, \ours~ has on average 0.0149 eV/\AA MAE on unseen 6-loop polymers, while on 5-loop and below the average MAE is 0.0117 eV/\AA.
In Figures~\ref{fig:static:natoms} and~\ref{fig:static:loop_size}, we present \ours's performance against polymer sizes. Linear regression analysis indicates that, on average, each increase of 100 atoms results in a significant increase of 5e-4 eV/\AA~in MAE. Notably, the model's performance on unseen polymers does not scale worse than on the seen polymers. In terms of loop sizes, we observe that the MAE for cycloalkanes remains stable as the loop number increases, while other polymer classes show a moderate increase. Overall, these results demonstrate that \ours~ extrapolates well to polymers of different sizes and unseen polymer types.

 \zc{ How about results on energy?  It will be good to put energy accuracy here. Remember to update the subsection heading to force and energy.} 
}

==> exp_sim_robust.tex <==

\subsection{MD Simulation Robustness}
\label{sec:exp:sim_robust}

In Section~\ref{sec:exp:sim}, we demonstrated the high accuracy of \ours~ in MD simulations for large polymers. In this subsection, we highlight an additional advantage of \ours~ compared to baseline models. Specifically, we show that even for small polymers, the baseline models without the multi-molecule training paradigm of \ours~ suffer from unstable simulations. These unstable simulations manifest as trajectories ``collapse'' during MD simulations, further indicating that the baseline models struggle to generalize well in noisy MD environments.



We define the ``breaking'' of a molecular dynamics trajectory as the point when the interatomic distances between atoms diverge from a stable distribution to infinity. Intuitively this happens when the molecule breaks apart into several parts irretrievably. The previous works that investigate previous state-of-the-art machine learning forcefields discovered that the trajectory can easily break apart even when the single snapshot accuracy of forces is high.~\cite{fu2022forces} In order to quantify this, we first define the interatomic distances at time \(t\) as \(\mathbf{D}_t\in\mathbf{R}^{n_a\times n_a}\) where the \(ij\) element corresponds to the distance between the \(i\)th and the \(j\) atom. Then denote \(\mathbf{S}_t = \Vert \mathbf{D}_t - \mathbf{D}_0\Vert_\infty\).
\(\mathbf{S}_t\) is an upper bound of the usual root mean squared deviation (RMSD) metric~\cite{fu2022forces,huan2017universal}. 
Intuitively, we measure how at time \(t\) the interatomic distances deviate from the starting conformation. \(\mathbf{S}_t\) is determined by the maximum deviation observed at time \(t\). Despite the initial increase due to the energy injection determined by the thermostat, in a stable MD simulation, \(\mathbf{S}_t\) should converge to a stable distribution. 
If \(\mathbf{S}_t\) increases continuously after a certain point \(T\), it means that the distances between at least one pair of atoms are behaving abnormally, indicating the ``breaking'' of the MD simulation. To quantify this we define the following statistics: 

\begin{equation}
    \begin{aligned}
        \mathbf{S}^*_t & = \max_{s\leq t} \log(\mathbf{S}_t), \\
        \nabla{\mathbf{S}}^*_t & = \begin{cases}
            1& \mathbf{S}^*_t - \mathbf{S}^*_{t-1} > 0, \\
            0,              & \mathrm{otherwise}
        \end{cases},  \\
        r_t & = \frac{\sum_{i=1}^{p} \nabla{\mathbf{S}}^*_i } { p },
    \end{aligned}
\end{equation}
for some \(p>0\). The scalar \(r_t\) evaluates the percentage of the number of snapshots after time \(t\) that keep deviating from a stable trajectory. We note that the simulation breaks whenever \(r_t\) becomes a constant 1 after a certain time \(T\). 

In Table~\ref{tab:sim_robustness_6loop}, the maximum number of steps before the trajectory exploded is reported. The baseline methods such as NequIP and TorchMDNet are trained exclusively on the single types of molecules for simulation. While in previous works~\cite{tholke2022torchmd,batzner20223} they have reported high accuracy forces in static evaluations, in simulations they collapse typically after a few tens or hundreds of thousands of steps. In practice, this is not enough for MD simulation purposes. \ours~ on the other hand, can produce robust simulations for these polymers. The observation is consistent as in Section~\ref{sec:exp:sim}, where \ours~ can run accurate and stable simulations for unseen large polymers. 

 \zc{ In addition to the table, it will be good to show several case studies. For the same 6 loop polymers, as some time step the baselines will just break the polymers, while our method  can still simulate robustly.} 


==> experiment.tex <==



\section{Results}
\newcommand{\widthere}{0.22}
\begin{figure*}[tp]
    \centering
    \subfigure[Forces Correlation for 15 Loop CK6.]{
        \includegraphics[width=\widthere\linewidth]{figs/large_995_12.png}
    }
    \subfigure[Forces Correlation for 15 Loop OTH4.]{
        \includegraphics[width=\widthere\linewidth]{figs/large_1053_12.png}
    }
        \subfigure[Forces Correlation for 15 Loop LAC2.]{
        \includegraphics[width=\widthere\linewidth]{figs/large_7_15.png}
    }
    \subfigure[Forces Correlation for 15 Loop LAC5.]{
        \includegraphics[width=\widthere\linewidth]{figs/large_1_15.png}
    }
    
    \subfigure[RMSD and Potential Energy for 15 Loop CK6.]{
        \includegraphics[width=\widthere\linewidth]{figs/large_995_12_rmsd_energy.png}
    }
    \subfigure[RMSD and Potential Energy for 15 Loop OTH4.]{
        \includegraphics[width=\widthere\linewidth]{figs/large_1053_12_rmsd_energy.png}
    }
    \subfigure[RMSD and Potential Energy for 15 Loop LAC2.]{
        \includegraphics[width=\widthere\linewidth]{figs/large_7_15_rmsd_energy.png}
    }
    \subfigure[RMSD and Potential Energy for 15 Loop LAC5.]{
        \includegraphics[width=\widthere\linewidth]{figs/large_1_15_rmsd_energy.png}
    }

    \subfigure[Dynamics Illustration for CK6.]{
        \includegraphics[width=\widthere\linewidth]{figs/995-illus.pdf}
    }
    \subfigure[Dynamics Illustration for OTH4.]{
        \includegraphics[width=\widthere\linewidth]{figs/1053-illus.pdf}
    }
    \subfigure[Dynamics Illustration for LAC2.]{
        \includegraphics[width=\widthere\linewidth]{figs/ID7-illus.pdf}
    }
    \subfigure[Dynamics Illustration for LAC5.]{
        \includegraphics[width=\widthere\linewidth]{figs/ID1-illus.pdf}
    }
    \caption{Accuracy and Robustness of \ours~ in MD simulations for large polymers. We select 15 loop CK6 (cycloctane), OTH4 (n-alkane substituted \(\delta\)-valerolactone), LAC2 (\(\gamma\)-butyrolactone) and LAC5 (3-methyl-1,4-dioxan-2-one) as examples. In (a)-(d) it is observed that \ours~forces are highly correlated with DFT forces during its own MD simulations. (e)-(h) shows the RMSD and potential energy curves of \ours~ during MD simulations. The curves suggest that \ours~simulations experience equilibration. (i)-(j) presents a visualization of sample conformations captured at various time points during the simulation process, which shows \ours could effectively explore and reveal the dynamic changes in polymer structures over time.}
    \label{fig:large_polymer}
\end{figure*}

%\subsection{Model Parameters and Training}

% We present the empirical validation results on ~\ours for polymer simulations and forces prediction. 
% First, we introduce the specifics of the model architecture and training details in Section~\ref{sec:exp_specifics}. 
% The general setting is that the model will be trained on smaller polymers of loop size \(5\) and less where we can employ DFT to generate large amounts of reference data efficiently. 
% In Section~\ref{sec:exp:sim} we experiment with 15-loop large polymers, which are 3 times the largest loop size the model has seen during training. 
% In Section~\ref{sec:exp:multimolecule}, we further analyze the multi-molecule forces prediction performance of \ours, showing that the ability to scale to training on diverse polymer families leads to improved performance and extrapolation ability. Section~\ref{sec:exp:sim_robust} shows that baseline deep learning forcefields suffer from simulation instability, further highlighting \ours~ advantage for MD simulations. 

We have conducted empirical validation on \ours ~for polymer simulations and
force prediction. We first provide details of the model architecture and
training in Section~\ref{sec:exp_specifics}. Specifically, we trained the
model on smaller polymers with a loop size of \(5\) or less, which were
generated by DFT efficiently. In Section~\ref{sec:exp:sim}, we test our
model on unseen larger polymers with 15 loops, which are three times larger than
the largest loop size used during training. Our results demonstrate the
scalability of \ours, as well as its ability to accurately predict forces
on larger polymers. In Section~\ref{sec:exp:multimolecule}, we further
analyze the performance of \ours~ in redicting forces on multiple polymer
families, showing that training on diverse polymer families can
improve the performance and extrapolation ability of \ours. Finally, in
Section~\ref{sec:exp:sim_robust}, we demonstrate that baseline deep
learning forcefields suffer from simulation instability, whereas \ours
performs MD simulations robustly.




\subsection{Experiment Setup}
\label{sec:exp_specifics}



\paragraph*{Baseline methods.}
We select state-of-the-art deep learning forcefields with Equivariant Graph Neural Network structures as baselines:  
\begin{enumerate}
    \item SchNet by~\citet{schutt2018schnet} which uses Graph Neural Network built on continuous convolutional layers for modeling the interatomic potentials, 
    \item NequIP by~\citet{batzner20223} that uses spherical harmonic based representations~\cite{thomas2018tensor,fuchs2020se} to build equivariant features for MD forcefield and simulations, 
    \item TorchMDNet by~\citet{tholke2022torchmd}, which similar to our method combines continuous convolutional layers and Equivariant Graph Neural Network~\cite{satorras2021n} for modeling  interatomic potentials.
\end{enumerate}
All of these methods are built on equivariant interatomic features and utilize different implementations of attention-based GNN layers for potential energy and forcefield prediction. In their papers, they have reported accurate forcefield prediction on MD17 dataset~\cite{chmiela2018towards}. %The forcefields in the papers are trained and evaluated separately on different molecules. 
 %\zc{ This sentence is vague. How do you train those models on our data set? Also single molecule settings?} 
In the papers on baseline methods, the models were trained and evaluated separately for different molecules. %The accuracy of forces in simulation settings was not reported in the papers.


\paragraph*{Model Architecture and Training.}
We implement a 6-layer Equivariant Transformer with an embedding dimension of 128 and 8 attention heads. In training, unless otherwise specified, the model is trained with 5-loop polymers and below. Polymers of size 6 and larger are unseen to the model during training and used as test data. 5\% of the training data is taken as the validation set. For each 500 training steps, the validation loss is recorded. 
We train the model with Adam optimizer for 3 epochs with \(0.0001\) initial learning rate, and the learning rate decays by a multiplicative factor of \(0.8\) whenever the validation loss increases for 30 consecutive validation steps. 

\input{exp_sim.tex}

\begin{figure*}[tp]
  \centering
  \begin{tabular}{ l c c}
  \multicolumn{3}{c}{\subfigure[ Violin plot of MAE of 4 methods trained reported on all types of polymers. ]{
    \includegraphics[width=.32\linewidth]{figs/naive_multimodel_mae.pdf}
    \label{fig:multimodel_mae} }
    } \\
    \hide{
    \hline
    \textbf{Method} & \textbf{MAE} & \textbf{Cosine Distance} \\
    \hline
    SchNet & 0.4796	& 0.2205 \\ 
    NequIP	& 0.0922	& 0.0156 \\
    TorchMDNet &	0.0421	 & 0.0038 \\ 
    DEPT	& 0.0073	& 8.67E-05 \\
    \multicolumn{3}{l}{\textbf{Averaged force error across all monomers in eV/\AA.  }}  
    }
  \end{tabular}%
  \begin{tabular}{ c c }
    \subfigure[SchNet]{\includegraphics[width=.29\linewidth]{figs/naive_multimodel_schnet_scatter.pdf}} &
      \subfigure[NequIP]{\includegraphics[width=.29\linewidth]{figs/naive_multimodel_nequip_scatter.pdf}} \\
    \subfigure[TorchMDNet]{\includegraphics[width=.29\linewidth]{figs/naive_multimodel_et_scatter.pdf}} &
      \subfigure[\ours]{\includegraphics[width=.29\linewidth]{figs/naive_multimodel_dept_scatter.pdf}}
  \end{tabular}
  \caption{Performance of deep learning forcefield, including SchNet, NequIP, TorchMDNet, and ~\ours~on multi-molecule training. Two metrics, Mean Absolute Error (MAE) and Cosine Distance (CosD) are reported. On the left, (a) shows the MAE comparison between models across 4 types of monomers: cycloalkanes, lactones, ethers, and others, as in Table~\ref{table:data}. On the right, (b) - (e) shows the scatter plots of DFT forces compared with predicted forces for the 4 methods. }
  \label{fig:multimodel}
\end{figure*}

\input{exp_monomer.tex}


\begin{figure*}[tp]
    \centering
    \subfigure[Multi-molecule vs. Single-molecule.]{
        \includegraphics[width=0.23\textwidth]{figs/single_multi_compare.pdf}
        \label{fig:static:single_multi}
    }
    \subfigure[Extrapolation to Unseen Polymers.]{
        \includegraphics[width=0.23\textwidth]{figs/seen_unseen.pdf}
        \label{fig:static:seen_unseen}
    }
    \subfigure[Extrapolation vs Polymer Size.]{
        \includegraphics[width=0.23\textwidth]{figs/seen_unseen_size.pdf}
        \label{fig:static:natoms}
    }
    \subfigure[Extrapolation vs Loop Sizes.]{
        \includegraphics[width=0.23\textwidth]{figs/seen_unseen_loop.pdf}
        \label{fig:static:loop_size}
    }
    \caption{Analyzing the performance of \ours. In Figure~\ref{fig:static:single_multi}, we compare the performance of models trained on single molecules and multiple molecules. \ours~ can uniformly improve forces accuracy by 10x times when trained on multiple molecules. Figure~\ref{fig:static:seen_unseen} analyzes \ours's extrapolation performance to polymers not seen during training. Figure~\ref{fig:static:natoms} and~\ref{fig:static:loop_size} show the performance vs the number of atoms and the loop sizes. }
    \label{fig:static_analysis}
\end{figure*}
\input{exp_sim_robust.tex}

%\subsection{Simulation Efficiency}


==> experiment_old.tex <==
\section{Experiments}

Following traditional evaluation metrics for machine learning forcefields, we first evaluate \ours~ on a static setting. Namely, \ours~ will be used to predict forces on fixed trajectories generated by DFT forcefield. This will evaluate how accurate the machine learning forcefield is on fixed molecular conformations generated by DFT which is assumed accurate and reliable.  
However, this setting is not realistic, as it is not an indicator of the forcefield's performance in a molecular dynamics simulation. 

Then we evaluate on a more realistic setting by testing the robustness and reliablility of \ours~ in molecular dynamics simulation.

\subsection{Static Forces Evaluation}
\label{sec:static_forces_eval}
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/static_forces_eval_mae.pdf}
        \caption{Mean Absolute Error.}
        \label{fig:static_mse}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/static_forces_eval_cosine.pdf}
        \caption{Cosine Similarity.}
        \label{fig:static_cosine}
    \end{subfigure}
    \caption{Mean Absolute Error (MAE) and Cosine Similarity (CS) between DFT and \ours~forces on static trajectories on molecules with \(\geq 75\) atoms. Molecules are sorted increasingly in the number of atoms from left to right. Each datapoint corresponds to the mean and standard deviation of MAE or CS of a molecule. The black points correspond to molecules that are included in the model's training samples, and green points correspond to molecules that are not seen by the model, which tests the model's ability to predict forces for unknown types of molecules on fixed conformations. For molecules seen by the model, the conformations are chosen from a trajectory not in the training set.} 
    \label{fig:static_forces}
\end{figure*}

\hide{
We report the ability of \ours~to predict accurate forces on fixed conformations. In Figure~\ref{fig:static_forces}, we visualize the mean absolute error and cosine similarity between \ours~predicted forces with DFT forces on DFT trajectories. For convenience of visualization, we showed only molecules with the numebr of atoms greater than or equal to 75. We note the following observations. Across all molecules, the mean MAE between \ours~and DFT forces is 0.0125 ev/\AA~with 0.0014 standard deviation. The cosine similarity and its standard deviation are 0.9996 and 0.0001. Furthermore, there is no statistical significantly difference between in-domain and off-domain molecules. 
We also compared the performance of \ours~with EGNN trained and evaluated exclusively on conformations of individual molecules. 
We observe a decrease of 0.0001 cosine similarity and an increase of 0.0053 increase in MAE on average for off-domain molecules. The decrease in performance is expected for the model attempting to capture way more information about atomic interactions in the same number of parameters in a single model, which is however small enough to ignore compared with the great benefit of an unified model that can be used accurately without training on off-domain molecules. 
}
In this study, we evaluate the accuracy of the \ours~model in predicting forces on fixed conformations. Figure~\ref{fig:static_forces} illustrates the mean absolute error (MAE) and cosine similarity between \ours~predicted forces and DFT forces on DFT trajectories. To simplify visualization, only molecules with a minimum of 75 atoms are displayed. Our findings show that across all molecules, the average MAE between \ours~and DFT forces is 0.0125 eV/Å with a standard deviation of 0.0014. The cosine similarity and its standard deviation are 0.9996 and 0.0001, respectively, with no statistically significant difference between in-domain and off-domain molecules.

We also compare the performance of \ours~with an EGNN model that was trained and evaluated exclusively on conformations of individual molecules. The results show a slight decrease in cosine similarity (0.0001) and increase in MAE (0.0053) on average for off-domain molecules. This decline in performance is expected, as the \ours~model has to capture more information about atomic interactions within the same number of parameters in a single model. However, the decrease is minor and outweighed by the benefits of having a unified model that can be used accurately without training on off-domain molecules.

\subsection{Dynamics Evaluation}
\hide{
In order to validate the model's ability to produce useful forces in actual molecular dynamics applications, we use our pretrained forcefield to generate molecular simulation trajectories on seen and unseen molecules. 
Most of the existing machine learning forcefield algorithms focus on evaluating the forces predicted by the models on static and in-domain molecular conformations, which is far from the real simulation scenario and not indicative of how the model would actually perform in a simulation setting. 
This is an important aspect of machine learning forcefields that existing state-of-the-art methods are not focused on for evaluation. As several papers have discovered \rui{reference}, the current state-of-the-art methods, while achiving high accuracy on forces prediction on single in-domain molecules, they fail drastically in simulation environments.
}
To demonstrate the practical utility of the model in real molecular dynamics applications, we use our pretrained forcefield to generate molecular simulation trajectories on both seen and unseen molecules. Unlike most machine learning forcefield algorithms, which only evaluate the forces predicted by the models on static, in-domain molecular conformations, our approach takes into account how the model would perform in a simulation setting.

This is a critical aspect that is often overlooked in the evaluation of machine learning forcefields. As previous studies have shown, state-of-the-art methods, while achieving high accuracy in predicting forces on single in-domain molecules, they can perform poorly in simulation environments. Thus, evaluating the performance of our forcefield in actual simulation scenarios provides valuable insights into its ability to produce useful forces in practical molecular dynamics applications.

To assess the reliability of a machine learning forcefield in simulation, we examine two key properties of the generated trajectory:

\begin{enumerate}
    \item \emph{Robustness}: This property reflects the stability of the trajectory in a realistic simulation environment. The molecule should maintain its integrity and converge to a stable conformation distribution, instead of breaking apart.
    \item \emph{Reliability}: This property determines the ability of the trajectory to accurately predict forces for molecules even after they deviate from their initial conformation distribution. The trajectory should remain reliable over time, even as the molecular conformations change during the simulation.
\end{enumerate}


For the robustness property, we define the ``breaking'' of a molecular dynamics trajectory as the point when the interatomic distances between atoms diverges from a stable distribution to infinity. Intuitively this happens when the molecule breaks apart into several parts irretrivably. The previous works that investigate previous state-of-the-art machine learning forcefields discovered that the trajectory can easily break apart even when the single snapshot accuracy of forces is high. In order to quantify this, we first define the interatomic distances at time \(t\) as \(\mathbf{D}_t\in\mathbf{R}^{n_a\times n_a}\) where the \(ij\) element corresponds to the distance between the \(i\)th and the \(j\) atom. Then denote \(\mathbf{S}_t = \Vert \mathbf{D}_t - \mathbf{D}_0\Vert_\infty\). Intuitively, we measure how at time \(t\) the conformation deviates from the original conformation at the start of the simulation. 
It is natural for \(\mathbf{D}_t\) to deviate from \(\mathbf{D}_0\) especially at the start of the simulation since the conformation would change according to the energy injection specified by different thermostats. However, we note that \(\mathbf{S}_t\) should converge to a stable distribution in a stable trajectory and the trajectory would break at time \(T\) when \(\mathbf{S}_t\) starts to monotonically increase for all \(t\) after \(T\). Based on this intuition we define
\begin{equation}
    \begin{aligned}
        \mathbf{S}^*_t & = \max_{s\leq t} \log(\mathbf{S}_t), \\
        \nabla{\mathbf{S}}^*_t & = \begin{cases}
            1& \mathbf{S}^*_t - \mathbf{S}^*_{t-1} > 0, \\
            0,              & \mathrm{otherwise}
        \end{cases},  \\
        r_t & = \frac{\sum_{i=1}^{p} \nabla{\mathbf{S}}^*_i } { p },
    \end{aligned}
\end{equation}
for some \(p>0\). The scalar \(r_t\) evaluates the percentage of the number snapshots after time \(t\) that keeps deviate from a stable trajectory. We note that the simulation breaks whenever \(r_t\) becomes a constant 1 after certain time \(T\). 

Simulation setting: ASE, Noose-Hover, 300k, 0.5fs, ...

We use 

\subsection{Comparing with Single-molecule EGNN}
\begin{figure*}
    \includegraphics[width=0.95
    \linewidth]{figs/6loop_single_forcefield.pdf}
    \caption{Single-molecule Equivariant Transformers in Simulation. We plot the RMSD curve along the simulation for 3 molecules and display the molecular conformations before and after the trajectory exploded. }
    \label{fig:six_loop_robustness}
\end{figure*}
In Section~\ref{sec:static_forces_eval} we noticed minimal performance drop for molecules using \ours~in comparison with single-molecule ET models. In this section, we further justify the benefit of \ours~in a simulation scenario. Although single-molecule ET could potentially achieve higher accuracy and correlation with DFT forces when evaluated on a given DFT trajectory as shown in ~\ref{fig:six_loop_robustness}. The figures show that the single-molecule ET models explodes after 60k, 100k, and 120k steps for C36H72, C60H108O12, and C84H156O12, respectively. However, \ours~can keep the simulation stable with a converged RMSD. The comparison shows that the static evaluation on fixed trajectories are not an indicator of how the model would perform in simulation. From a machine learning perspective, the model trained and evaluated on a single molecule would overfit to a small region of distribution of conformations. In a simulation environment, such models are prone to encounter a conformation with which the model has high uncertainty, leading to higher errors that trigger the trajectory to explode. 

\subsection{Generalization to Larger Molecules}
One of the major bottleneck of previous deep learning forcefield is generalization to larger molecular structures. As the DFT forces scale nearly as \(O(N^7)\) to the number of atoms, efficient forcefield that can be accurately generalized to large molecular systems is essential. 

We test on the following molecular systems: 

These molecules are built on the same monomers that are present in the training set, but repeated for \(12\) and \(15\)-loops. As the largest number of loops in the training data of \ours~is 5-loop, we are testing \ours~ on unseen molecules 2-3 times the size that the model is familiar with in the training set. 

We report 0.9999 cosine similarity that is statistically almost identical as the generalization performance to 6-loop. When molecule sizes increases in a known molecular family, \ours~performance is not hindered by the molecule size increase or the noise introduced in the simulation environment. 

\label{fig:large_mol_dft}
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/995_12_dft_compare.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/995_15_dft_compare.pdf}
    \end{subfigure}
\end{figure*}

\subsection{Generalization to New Molecular Structures} 

\subsubsection{Aspirin}
In this experiment, we test our model on public molecules with popular deep learning forcefields. 
\begin{itemize}
    \item TorchMD-Net~\cite{tholke2022torchmd} is a deep learning architecture designed for molecular dynamics. Similar to our approach, it uses deep equivariant transformers to learn machine learning potentials for single molecules. 
    \item GemNet~\cite{gasteiger2021gemnet} is a type of equivariant graph neural network for learning molecular representations. We use both pretrained GemNET and finetune it on the specific molecules and GemNET trained on the molecules from scratch. 
    \item Nequip~\cite{satorras2021n} is a type of SE(3)-Transformer used for molecular dynamics. Compared with TorchMD-Net and GemNet, Nequip is more principled in modeling the equivariant actions on high-dimensional hidden spaces at the cost of computation efficiency. 
\end{itemize}

We report that on Aspirin, these methods explode after ... . However, our method runs for 1000k steps before eventually the trajectory explodes. 

Aspirin contains a benzene ring, which is a molecular structure unseen in any of our dataset. However, in simulation, our model can keep the benzene ring structure for a long time before explosion. While the model has certain generalization ability to different molecular structures, the uncertainty brought by a new structure still accumulates to the point that triggers the explosion. 


\subsection{Model Efficiency}

==> intro.tex <==
\section{Introduction}

%Molecular dynamics is a valuable tool for analyzing chemical reactions and properties of molecules while learning accurate and efficient forcefield for molecular dynamics remains a challenge and an active research field. 
%The more accurate methods for molecular dynamics are \emph{ab initio} methods, which is a class of principled methods in quantum chemistry capable of solving Schr\"odinger's equation for complex molecular systems. However, they are still relatively costly for large molecules. For example, a popular method, \emph{Density Function Theory} (DFT), has a time complexity of \(O(N^3)\) where \(N\) is the number of atoms. CCSD(T), while being more accurate, has \(O(N^3)\). For a complex molecule system such as one with hundreds of atoms, the computation could take hours and a sufficiently large dataset could take weeks if not months. 

%Developing efficient and accurate forcefield for molecules is one of the central problems in computational chemistry.
%Forces are defined as the partial derivative of the potential energy of a molecule with respect to the atom positions and provide the acceleration of atomic positions. 
%They provide valuable information on the behavior of atoms and molecules in different environments. 
%An accurate forcefield is essential to many applications in computational chemistry, such as 
%    molecular dynamics simulation,
%    conformation optimization, 
%    property prediction,
%    reaction prediction, and 
%    drug discovery. 
%Traditional approaches in computational chemistry developing forcefields face a tradeoff between accuracy and efficiency. For example, \emph{ab init} (``from the first principle'') methods, such as the family of \emph{DFT} methods, represent principled and most accurate forcefield that are obtained by solving approximations of the Shr\"odinger's equation that govern the quantum behavior of atoms. However, \emph{DFT} has a time complexity of \(O(N^3)\) where \(N\) is the number of electrons. Empirically this is \(O(N^7)\) in terms of the number of atoms, making them unscalable to large molecule systems. 
%In computational chemistry literature, classifical forcefields represent a faster line of methods that fit empirical energy equations from handcrafted atomistic features. These methods are much faster but less accurate.

% maybe a brief summary to unite the following two paragraphs? this paper focuses on ... . the two ingredients are ... . 

% first: machine learning forcefield overview

Molecular dynamics (MD) is a computer simulation method used to study the physical movements of molecules and the interactions between them. It is an important tool in the field of computational chemistry and materials science, as it allows scientists and engineers to study the behavior of complex molecular systems under various conditions and predict 

The word ``dynamics'' in MD refers to Newton's second law, which determines how the ``classical'' systems evolves in the space and time. In short, the force exerting on each atom at a given time creates an acceleration, changing the velocity and the atoms, and ultimately governing all the atoms and the whole system. Therefore, rapidly and accurately computing the atomic forces is very important for MD simulations.

In recent years, there's been active research in developing machine learning forcefields. Generally, these methods build on equivariant graph neural networks~\citep{scarselli2008graph,zhou2020graph}, message passing frameworks~\citep{klicpera2020directional,gilmer2017neural}, or tensor field networks~\citep{thomas2018tensor,fuchs2020se,batzner20223,geiger2022e3nn}
to model the interatomic relations in molecules. To guarantee energy conservation, these models predict the potential energy of molecules, then obtain the forces by the partial derivative of the potential energy w.r.t.\ atomic positions. 
Usually, they train on the empirical energy and forces generated by accurate but inefficient methods such as Density-functional theory (\emph{DFT}) in computational chemistry. By leveraging the parallelization capacity of modern GPU, deep neural networks are hopeful to achieve accuracy close to DFT with reasonable computation time. 

% second: pretraining. 
Self-supervised pretraining techniques have proved to be effective in learning representations in natural language processing, computer vision, and graphs. Generally, they employ self-supervised learning methods to encode prior information in the pretrained models and the representations of data. 
Motivated by graph pretraining, there have been works on pretraining on molecular graphs~\cite{zaidi2022pre,liu2021pre,zhu2021dual}. However, empirical findings~\cite{sun2022does} suggest that these pretraining techniques derived from popular strategies for graph pretraining have limited improvement over untrained models. We speculate that 3D molecules are fundamentally different than 2D graph structures and require specific supervised pretraining approaches~\cite{gao2022supervised}.

% limitations.
Despite recent advances in ML forcefield, a few key elements that are required for successful and reliable application of such forcefield for molecular dynamics are missing. 
First, the ML forcefield needs to be able to train on and predict multiple molecule systems. We want a unified forcefield that can handle a class of molecules, instead of having to train and store a new model whenever there is a need to modify the molecular structure. Second, the model needs to be able to generalize to unseen molecules, especially from smaller systems to larger ones. The computation bottleneck for accurate \emph{ab init} forcefield dictates that we would have a relatively large amount of small molecules, but larger molecules would be scarce. It is of great importance to be able to reliably generalize to larger molecules for simulations. 
Third, the simulations that run on ML forcefields need to be stable. During a molecular dynamics simulation, the molecule evolves and accumulates noise, and eventually could lead to \emph{out-of-distribution} situations where machine learning models are known to be unstable. Indeed, \citet{fu2022forces} [and another paper] suggest that state-of-the-art ML forcefields are unable to maintain stability in long-term simulations. 
%First, the ML forcefield needs to be generalizable to unseen types of molecules. In application, the researchers usually want to experiment on multiple variants of similar molecular structures. Existing methods train and evaluate on single molecule types, and perform poorly in terms of generalization ability. Typically, they only train on 1000 conformations from a single type of small molecule~\cite{tholke2022torchmd,schutt2018schnet,klicpera2020directional,batzner20223} and is easily overfit to a small data region. 
%Second, the ML forcefield needs to be 

We find that the current state-of-the-art papers on ML forcefield emphasize on small-scale evaluation of static and small molecular conformations that do not align with the practical needs mentioned above. Most of the existing ML forcefield train and evaluate on small dataset from individual small molecules~\cite{tholke2022torchmd,schutt2018schnet,klicpera2020directional,batzner20223}. This lack of diversity in training and evaluation is what we suspect one major hindrance in practicality, preventing them from being generalizable and robust in simulations. We empirically show that [ref to paper] these methods can't be trained on the energy and forces on multiple molecules efficiently. 
On the other hand, while pretraining methods have become one of the most effective tools for learning universal and transferable models, blindly applying them without consideration of the idiosyncrasies of molecular systems has dubious effects, as we empirically found in [ref to paper], inline with previous findings~\cite{sun2022does}.



% pretraining wouldn't work without forces. Theoretically analyze it. 

% 1. the source of data. DFT - only small molecules. 
% 2. Not generalizable. Only single molecule systems. 
% 3. Unreliable dynamics. 
% 4. Pretraining doesn't work.


% we argue that forces. 

%This paper investigates the generalization of machine learning forcefields to large molecules with minimal or no training data. Generalization of machine learning forcefield is a challenging task, as different molecules have drastically different internal dynamics. To date, most of the existing machine learning approaches assume ample data on a single, typically small molecule. 
%In authentic applications in chemical or material science, however, the model needs to be able to predict accurate energy and forcefield for unseen large molecules for efficient estimation of their properties. Existing methods that are only trained for single small molecules cannot be used in these applications. 
In this paper, we develop a unified large-scale pretrained model for general forcefield prediction. To facilitate this, we develop a forcefield prediction model that can take advantage of large data of molecules and learn from the different internal mechanics of diversified molecular structures. There are several advantages to doing this. First, by learning a general model on large data, the model is able to predict more accurate forcefields compared with models trained on small amounts of molecule configurations from single sources. 
Second, as the model is able to learn the mechanics of forcefield prediction more robustly across forcefields, it can generate accurate and reliable forcefield prediction for unseen molecules as well, while existing machine learning forcefield approaches may fail catastrophically for unseen molecules or in multi-molecule prediction settings. With an accurate and reliable forcefield, our model can be put to more practical applications of approximating molecular dynamics efficiently, which is  needed typically for large unknown molecules that are ineffective to approximate with \textit{ab init} methods. 

%Recent advances inspire our work in pretrained models in Natural Language Processing and Graphs. In the recent development of machine learning, researchers have discovered the efficacy of pre-trained models on extensive unlabeled data in generalization or fast adaptation to downstream tasks, such as in natural language processing, image processing, and graphs. 
%Typically, in this paradigm, one trains a large-scale universal pretrained model that is trained on large unlabeled data. The pretrained models are believed to produce potent representations for data that allow for fast transfer to new tasks with a minimal finetuning process.
%\rui{examples} For example, in natural language processing, a line of work such as BERT, RoBERTa, and BART, train self-attention-based Transformers to capture the internal language structures from an astronomical amount of text from diversified sources. These models prove to be state-of-the-art in many NLP applications. 
%For machine learning for graphs, there have been advances in Graph Neural Networks, graph Transformers, etc. that allow the learning of graph structures for downstream tasks that rely on graph topology. However, pretraining in graphs has not achieved such popularity, since \rui{why} 
% unlike languages that share the same fundamental structure, graphs in different applications don't necessarily share the same topological structures.  

%In the field of machine learning forcefield, however, we can expect successful pretrained models with graphs. In molecular dynamics, we deal with molecules represented in their 3D coordinates, which can be naturally represented as graphs, with atoms being graph nodes, and distances between atoms being edges. Furthermore, the molecule graphs can also encode the 3D structures by giving graph nodes their 3D coordinates. 
%We can have a large collection of molecules of diversified structures and mechanics, but fundamentally they behave according to the same physical and chemical principles. This, and the potent representation capability of deep Equivariant Graph Neural Network Models and self-attention-based Transformers, has enabled us to pack the knowledge of a large collection of molecules in a deep model for unified forcefield training. 



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> method.tex <==

\input{method_paradigm.tex}
\input{method_et.tex}

==> method_et.tex <==
\section{Equivariant Transformers}
\label{sec:transformer}

%In order to learn the complex quantum mechanical interactions between atoms for accurate forcefields for varying types of polymers, we use Equivariant Transformers~\cite{tholke2022torchmd}
In this section, we introduce Equivariant Transformer~\cite{tholke2022torchmd} for learning polymer representations. We use the powerful \emph{attention mechanism}~\cite{vaswani2017attention} to model the interatomic potentials, where atoms learn the attraction-repulsion dynamics on relevant atoms in the molecule. Equivariant Transformer specifically adopts the Transformer architecture for molecular data, where the model computation process is required to be equivariant to the input molecules. 
While in general our training framework can apply to any machine learning forcefield model, we choose Equivariant Transformer~\cite{tholke2022torchmd} for the efficiency and expressivity of the Transformer architecture.

The Equivariant Transformer architecture operates on molecular data in the form of graphs and consists of three main blocks: an embedding layer, an updated layer, and an output network. 


\paragraph*{Embedding Layer}
The first component is an atom embedding layer, which transforms atoms to vector representations that encode the quantum mechanical information about the atoms and their surroundings. The atom embedding is further split to \emph{scalar} embeddings \(\mathbf{h}_0\in\RR^D\) and \emph{vector} embeddings \(\mathbf{v}_0\in\RR^{3\times D}\), where \(D\) is the embedding size. 
 The scalar embedding is derived by integrating both the intrinsic vector, which captures information specific to the atoms themselves, and the neighborhood vector, which encapsulates the interactions within the atomic neighborhoods. The intrinsic vector, denoted as \(\mathbf{x}^\mathrm{int}\), is acquired by associating each atom type with a corresponding dense feature vector in \(\RR^D\). To compute the neighborhood embedding \(\mathbf{x}^\mathrm{nbr}\), we initially define the distance filter using a radial basis function. Subsequently, a continuous-filter convolution technique is employed to aggregate information from the surrounding atoms within a given neighborhood. 
The atom embedding \(\mathbf{x}\) is obtained by the concatenation of intrinsic and neighborhood embeddings. 
The vector embedding \(\mathbf{v}\) is initialized as zero vectors in \(\RR^{3\times D}\). 


\paragraph*{Update Layers}
The update layers defines the incremental change of the \emph{scalar embeddings} \(\mathbf{x}\) and \emph{vector embeddings} \(\mathbf{v}\) in each network layer. For each atom \(i\), the update layers are defined as follows:
\begin{equation}
    \begin{aligned}
        \nabla \mathbf{x}_i & = f^{x}(\mathbf{x}_i) + \sum_{j} \phi^x(\mathbf{x}_i, \mathbf{x}_j) + \psi^{xv}(\mathbf{v}_i) \\ 
        \nabla \mathbf{v}_i & = f^{v}(\mathbf{v}_i) + \sum_{j} \frac{\mathbf{r}_j - \mathbf{r}_i}{\Vert \mathbf{r}_j - \mathbf{r}_i\Vert} \phi^{v}(\mathbf{x}_i, \mathbf{x}_j) + \psi^{vx}(\mathbf{x}_i).
    \end{aligned}
\end{equation}
For each atom \(i\), the attention mechanism \(phi^x\) and \(\phi^v\) will model its interatomic potentials to all other atoms. Based on the embeddings of two atoms and their relative distance vectors, \(\phi^x\) and \(\phi^v\) defines the interaction between the two atoms. 
\(f^x\) and \(f^v\) are the residual connections~\cite{he2016identity} that prevents deep neural network architectures to suffer from performance degradation.
\(\psi^{xv}\) and \(\phi^{vx}\) defines the information excahnge between \(\mathbf{x}\) and \(\mathbf{v}\) in each layer. \(\psi^{xv}\) is used to update the vector embedding \(\mathbf{v}\) from the scalar embedding \(\mathbf{x}\), and \(\psi^{vx}\) is used to update the scalar embedding \(\mathbf{x}\) from the vector embedding \(\mathbf{v}\). 

\paragraph*{Output Network}
The output network computes scalar atom-wise predictions using gated equivariant blocks, which is a modified version of the gated residual network~\cite{tholke2022torchmd}. The gated equivariant blocks aggregate the atomic embeddings into a single molecular prediction. This prediction can be matched with a scalar target variable or differentiated against atomic coordinates to provide force predictions.


==> method_et__Rui_Feng_s_conflicted_copy_2023-04-23_.tex <==
\section{Equivariant Transformers}
\label{sec:transformer}

%In order to learn the complex quantum mechanical interactions between atoms for accurate forcefields for varying types of polymers, we use Equivariant Transformers~\cite{tholke2022torchmd}
In this section, we introduce Equivariant Transformer~\cite{tholke2022torchmd} for learning polymer representations. We use the powerful \emph{attention mechanism}~\cite{vaswani2017attention} to model the interatomic potentials, where atoms learn the attraction-repulsion dynamics on relevant atoms in the molecule. Equivariant Transformer specifically adopts the Transformer architecture for molecular data, where the model computation process is required to be equivariant to the input molecules. 
While in general our training framework can apply to any machine learning forcefield model, we choose Equivariant Transformer~\cite{tholke2022torchmd} for the efficiency and expressivity of the Transformer architecture.

The Equivariant Transformer architecture operates on molecular data in the form of graphs and consists of three main blocks: an embedding layer, an updated layer, and an output network. 


\paragraph*{Embedding Layer}
The first component is an atom embedding layer, which transforms atoms to vector representations that encode the quantum mechanical information about the atoms and their surroundings. The atom embedding is further split to \emph{scalar} embeddings \(\mathbf{h}_0\in\RR^D\) and \emph{vector} embeddings \(\mathbf{v}_0\in\RR^{3\times D}\), where \(D\) is the embedding size. 
 The scalar embedding is derived by integrating both the intrinsic vector, which captures information specific to the atoms themselves, and the neighborhood vector, which encapsulates the interactions within the atomic neighborhoods. The intrinsic vector, denoted as \(\mathbf{x}^\mathrm{int}\), is acquired by associating each atom type with a corresponding dense feature vector in \(\RR^D\). To compute the neighborhood embedding \(\mathbf{x}^\mathrm{nbr}\), we initially define the distance filter using a radial basis function. Subsequently, a continuous-filter convolution technique is employed to aggregate information from the surrounding atoms within a given neighborhood. 
The atom embedding \(\mathbf{x}\) is obtained by the concatenation of intrinsic and neighborhood embeddings. 
The vector embedding \(\mathbf{v}\) is initialized as zero vectors in \(\RR^{3\times D}\). 


\paragraph*{Update Layers}
\hide{The update layers define the interaction between atoms and between scalar and vector embeddings. 
The update layers compute interactions between pairs of atoms using a modified multi-head attention mechanism, updating the latent atomic representations.  The key component of the update layer is the \emph{modified attention mechanism}, which models the interatomic relations as follows:
\[
a_{ij} = \mathrm{dot}(Q_i, K_j, D_{ij}) \phi(d_{ij})
\]
where \(Q_i = W^Q \mathbf{x}_i, K_j = W^K \mathbf{x}_j\), \(D_{ij}\) is a distance filter on the distances between \(x_i\) and \(x_j\), and \(\phi(d_{ij}\) is the cutoff function. \(\mathrm{dot}\) represents a three-way dot product where \(\mathrm{dot}(x, y, z) = \sum x\circ y \circ z\). \(a_{ij}\) represents the attraction-repulsion states between atoms \(i, j\) which depends on the interatomic potential based on the latent atomic representations and the interatomic distances encoded in \(D^K\).
Then, the aggregated feature vector is \(y_i = \sum_{j=1}^N a_{ij} s_{ij}\)}

The update layers can be expressed as follows:
\begin{equation}
    \begin{aligned}
        \nabla \mathbf{x}_i & = f^{x}(\mathbf{x}_i) + \sum_{j} \phi^x(\mathbf{x}_i, \mathbf{x}_j) + \psi^{xv}(\mathbf{v}_i) \\ 
        \nabla \mathbf{v}_i & = f^{v}(\mathbf{v}_i) + \sum_{j} \frac{\mathbf{r}_j - \mathbf{r}_i}{\Vert \mathbf{r}_j - \mathbf{r}_i\Vert} \phi^{v}(\mathbf{x}_i, \mathbf{x}_j) + \psi^{vx}(\mathbf{x}_i)
    \end{aligned}
\end{equation}
which defines the incremental change of the \emph{scalar embeddings} \(\mathbf{x} in each network layer. \(\phi^x\) and \(\phi^v\) defines the attention mechanism between atoms. For each atom \(i\), the attention mechanism will model its interatomic potentials to all other atoms. 
\(f^x\) and \(f^v\) are the residual connections~\cite{he2016identity} that prevents deep neural network architectures to suffer from performance degradation.
\(\psi^{xv}\) and \(\phi^{vx}\) defines the information excahnge between \(\mathbf{x}\) and \(\mathbf{v}\) in each layer. \(\psi^{xv}\) is used to update the vector embedding \(\mathbf{v}\) from the scalar embedding \(\mathbf{x}\), and \(\psi^{vx}\) is used to update the scalar embedding \(\mathbf{x}\) from the vector embedding \(\mathbf{v}\). 

\paragraph*{Output Network}
The output network computes scalar atom-wise predictions using gated equivariant blocks, which is a modified version of the gated residual network~\cite{tholke2022torchmd}. The gated equivariant blocks aggregate the atomic embeddings into a single molecular prediction. This prediction can be matched with a scalar target variable or differentiated against atomic coordinates to provide force predictions.


==> method_old.tex <==


\section{General-forcefield Equivariant Graph Neural Network} 

We represent the coordinates of a molecular configuration as \(\mathbf{x} \in \mathbb{R}^{n_{a}\times 3}\) where \(n_a\) is the number of atoms in the molecule. 

Our goal is to develop a machine learning algorithm denoted by \(\Phi_\theta: \mathbf{x}\rightarrow (E, F)\) where \(E\) represents the potential energy of the molecule and \(F\) represents the forces. 
Motivated by works of ~\cite{schutt2018schnet,satorras2021n,tholke2022torchmd}, we implement an Equivariant Graph Neural Network (EGNN) that can effectively learn equivariant representations of molecules for the prediction of forces. 

Suppose the EGNN is denoted as \(\Phi_\theta\), we obtain the forces of a molecule by 
\begin{equation}
    \frac{\partial}{\partial{\mathbf{x}}}\Phi_\theta(\mathbf{x})
\end{equation}

where \(\Phi_\theta(\mathbf{x})\) outputs the potential energy of the molecular conformation \(\mathbf{x}\), 

The desired algorithm must satisfy the following conditions in order to produce chemically and physically feasible potential energy surface and forces: 1) equivariance w.r.t. the roto-translation actions in S(3) group, which means the following must be true given \(g\in S(3)\): 
\(\Phi_\theta \circ g (\mathbf{x}) \rightarrow (E, g(F))\). 2) law of conservation of energy, which can be satsified by letting \(F = - \frac{\partial E}{\partial \mathbf{x}}\). 

Existing works~\cite{schutt2018schnet,satorras2021n,tholke2022torchmd} focus extensively on single-molecule systems, which means that the models will be trained and evaluated on static trajectories of a single molecule. 
Two major shortcomings come with their training and evaluation scheme. Firstly, their model is not able to generalize to new molecular systems, even if they contain known atom types and similar molecular structures. Secondly, their model is not able to perform well in a realistic molecular dynamics simulation. 
In order to solve these issues, we 1) use a equivariant graph neural network that is able to learn rich interatomic potentials, and 2) pretrain it in a large variety of molecular families with a huge amount of data. Then, we are able to develop a model that can be generated to new and much more complicated molecular structures in realistic simulation settings. 



\subsection{Pretraining}
As opposed to existing single-molecule training frameworks, we propose a \emph{General-Forcefield Molecular Transformers} (\ours), where the model is \emph{pretrained} on forces of a diverse family of molecules of varying sizes. 

Mainstream machine learning forcefield optimize their parameters to find the minima of 
\[
    \mathbf{E}_{\mathbf{x}|T}\left[ \Vert \Phi_\theta(\mathbf{x}) - E \Vert + \left\Vert \frac{\Phi_\theta(\mathbf{x})}{\mathbf{x}} - F \right\Vert \right], 
\]
where \(\mathbf{x}|T\) describes the sample distribution of a given trajectory under certain fixed thermostat. There are two main obstacles in this objective. Firstly, the joint optimization of energy and forces is difficult and even untrainable, especially when multiple molecules are concerned. This makes the trained model unstable in simulation and hard to scale to multi-molecule settings, and making generalization to unseen molecules infeasible. Furthermore, the model parameters are optimized on a single fixed trajectory of a single molecule, undermining the model's robustness in real simulations. 

Classical forcefield bypass these problems by using physiochemistrical functionals that approximate the potential energy surface with prior physical knowledge. While with such knowledge can help learning the energy and forces with certain classes of molecular structures, no general approximation form could exist for arbitrary molecular structures. We therefore do not limit our model to fit certain approximation form of the potential energy, but instead utilize the rich representation ability of deep Transformers to learn more universal forcefields. 

Therefore, we optimize the following objective: 
\[
   \mathbf{E}_T\left[\mathbf{E}_{\mathbf{x}|T}\left[  \left\Vert \frac{\Phi_\theta(\mathbf{x})}{\mathbf{x}} - F \right\Vert \right]\right],
\]
where we addressed the two aformentioned drawbacks in previous objectives. 
The model parameters are optimized to predict forces. The rationale behind this design is that atomic forces are a more reliable and generalizable objective given by DFT calculations than the potential energy. The potential energy, defined on the molecule level, gives little information on the atomic level free energies. 
Empirically, forces are statistically of the same distribution in molecules, while energy distributions vary greatly, even after normalized by the number of atoms. 
In addition to training on forces, our objective takes into account of the distributional variations in different trajectories of the same distribution. And because of our objective is compatible of multi-molecule training, we can train on various molecule families with different sizes, 
allowing the model to learn from more possibilities of atomic interactions and how they change according to the molecule size.

We argue that our model does not lose information on the potential energy during simulation. The model trained in this manner produces output that is linearly correlated with the ground-truth energy, since both are defined as the integrals of the forces. 


%In comparison to the mainstream machine learning forcefield settings, our model is pretrained on the forces of the molecules only. 


\subsection{Simulation}
In the simulation stage, we use \ours~to generate forces for molecules on the fly. Since the model is only trained on forces, we need to obtain the energy during the simulation stage. 
The model output \(E^*(\mathbf{x})=\Phi_\theta(\mathbf{x})\) is linearly correlated with \(E(\mathbf{x})\)  

\subsection{Deep Interatomic Potential with Equivariant Transformers}
We model the interaction between atoms with a deep Equivariant Transformers (ET) model~\cite{tholke2022torchmd}. ET represents molecules as inputs by encoding the molecular structures into a compact and expressive representation known as a molecular embedding. 

\subsubsection{Equivariant Attention between Atoms}
The attention mechanism is a key component of the equivariant transformer architecture that enables it to efficiently encode molecular structures into molecular embeddings.

In the attention mechanism, the atomic features are used to compute pairwise attention scores between all pairs of atoms in the molecule. These attention scores indicate the relative importance of each pair of atoms in determining the overall molecular structure, and they are used to weigh the contributions of each atom to the final molecular embedding.

To ensure that the attention mechanism is equivariant to rotations and translations, the attention scores are computed using a radial basis function that takes into account the distances between atoms in the molecular structure. This allows the attention mechanism to capture the underlying physics of molecular interactions, such as electrostatic attraction and repulsion between atoms.

The attention scores are then used to compute a weighted sum of the features of each atom, which forms the final molecular embedding. 

\hide{
\begin{table}[]
    \centering
    \begin{tabular}{c|cccccc}
         & Cyclopropane & Cyclobutane & Cyclopentane & Cyclohexane & Cycloheptane \\
        Formula  & C3H6 & C4H8 & C5H10 & C6H12 & C7H14 \\
       \# Atoms  & 9 & 12 & 15 & 18 & 21 \\
      Model  & \includegraphics[width=0.1\textwidth]{pics/molecules/propane.png} 
        &  \includegraphics[width=0.1\textwidth]{pics/molecules/butane.png}
        &  \includegraphics[width=0.1\textwidth]{pics/molecules/pentane.png}
        &  \includegraphics[width=0.1\textwidth]{pics/molecules/hexane.png}
        & \includegraphics[width=0.1\textwidth]{pics/molecules/heptane.png}
    \end{tabular}
    \caption{Cycloalkane families used in experiments.}
    \label{tab:cyclo_alkane_data}
\end{table}
}

==> method_old_old.tex <==



\section{Method}

In this section, we develop our machine learning model to predict forcefield. We use a graph to represent a molecular conformation 
\(
G=(V, E)
\), where \(V\) is the set of atoms \(v_1,\ldots, v_N\), associated with 3D coordinates \(r_1, \ldots, r_N\) and atom types \(a_1,\ldots, a_N\). The goal of this section is to develop a model \(f:\mathbb{R}^{N\times 3} \rightarrow \mathbb{R}\) that satisfies the following:
\begin{equation}
\begin{aligned}
        f(\mathbf{x}; G) & = E \in \mathbb{R} \\
        \frac{d}{d\mathbf{x}}f & = F \in \mathbb{R}^{N\times 3}
\end{aligned}
\end{equation}
i.e. the model \(f\) takes atomic positions as input and outputs the \emph{potential energy} of the function. The gradient of the potential energy should be the forcefield. 
Furthermore, the model should satisfy \emph{equivariant} under \(SO(3)\), i.e. equivariant to the rotational, translational, and permutation operations in \(\mathbb{R}^3\). This is a basic physical constraint for any model applied to molecular property prediction, 
%since the rotation, translation and permutation of atoms in the atoms should not change the potential energy, and should change the atomic forcefield accordingly. 
since under rotation, translation, and permutation operations on atoms, the potential energy should always stay constant and the forcefield should change accordingly. 

%In order to efficiently model molecular dynamics, we model the inte
It is theorized that \rui{ask for ref} the potential energy of molecule conformations can be modeled by interactive atomic potentials, i.e. the relations between the atoms. Classical fingerprinting approaches features interactive atomic potentials by manually defining features by transforming the distances and angles between pairs of atoms. In this approach, on top of the distance features between atoms  (section~\ref{sec:distance_features}) that prove to effectively learn the interactions between atoms, we build self-attention modules( section~\ref{sec:self-attention}) that prove to effectively transform and learn more complex \emph{atomic embeddings} utilizing the interaction between atoms in a high dimensional space.

Furthermore, we model \emph{Latent 3D States} (section~\ref{sec:latent_3d_features}) for the 3d structures of molecules. Essentially, unlike data in typical machine learning applications such as NLP and CV, molecular structures lie explicitly in a 3-dimensional space. To model this defining feature of molecules, we initialize \emph{latent 3-dimensional states} for atom positions that interact with the atom embeddings via \emph{cross-attention mechanism}. This module better represents the 3-dimensional nature of molecules and prove to improve the performance of forcefield prediction. 

In Section~\ref{sec:optim} we introduce how our model is optimized by minimizing the mean squared error of forcefield prediction using Adam optimizer. 

\subsection{Distance features}
\label{sec:distance_features}
We use \({r}_{ij}\) to represent the distance between atom \(i\) and \(j\). 

\subsection{Self-Attention Module}
\label{sec:self-attention}


\subsection{Latent 3D States}
\label{sec:latent_3d_features}

\subsection{Optimization}
\label{sec:optim}

\subsection{Training}
\label{sec:training}


==> method_paradigm.tex <==
\section{\ours: A Generalized Training Paradigm for Machine Learning Polymers}
\label{sec:paradigm}
%We represent a molecule configuration as \(x=(\molconf, \atomtypes)\). \(\molconf\in\RR^{n_a}\), \(n_a\) being the number of atoms in the molecule, represents the 3D coordinates of atoms. \(\atomtypes\in\NN^{n_a}\) represents the atomic numbers of the atoms. 
%In this paper, we are concerned with two states of the molecule configuration, its potential energy \(E_x\in\RR\) and forces \(F_x\in\RR^{n_a\times 3}\). 
%In a MD simulation trajectory \(\thermo_x\), the molecule configurations are distributed according to the thermostat of the simulation. We denote the molecule distribution given trajectory as \(\molconf|\thermo_x\). 

\hide{\paragraph*{Notations.}
We represent a molecule as \(x\). Assuming \(n_x\) is the number of atoms, we represent the distribution of its conformations as \(\mathbf{r}_x\in \RR^{n_x\times 2}\) and the atom types of the molecule as \(\mathbf{z}_x\in \RR^{n_x}\). The potential energy of a molecule is determined given the conformation \(\mathbf{r}\sim\mathbf{r}_x\) and atom types, denoted as \(E=E(\mathbf{r}, \mathbf{z})\in\RR\). The forces applied on the atoms are obtained by \(F=-\frac{\partial E}{\partial \mathbf{r}}\in\RR^{n_x\times 3}\). In theory, a stable conformation is one where the potential energy achieves local minimum with zero forces. In MD simulations, the molecular conformations are moved according to forces and the thermostat of the simulation. Given an initial conformation \(\mathbf{r}_0\), we can denote the distribution of the conformation in a \emph{ab-initio}-based MD simulation given a certain thermostat \(\thermo\) as 
\(\mathbb{T}(x, \mathbf{r}_-1, \thermo)\). Because of the energy injection in the simulation, the conformations from this distribution are likely equipped with non-zero forces. 

\rui{change of structure here:}
\rui{our objective. rationale. how could it achieve large scale multi molecule? }
\rui{briefly, previous objective; major differences. }
}

%\subsection{Key Solution: Equivariant Transformer-based Forcefield for Multiple Molecule Training}

To solve the two problems, the key solution is to scale the model to parameterize forcefields for multiple molecules. If this is achieved, then the model will be hoping to a) implicitly learn the transferable quantum mechanics underlying different molecules, leading to better generalization ability; and b) handle the more diverse conformations in simulation environments, as the model has seen more types of quantum interactions between atoms. 
To be able to achieve these, the model will need to have strong representation ability. 
Inspired by recent successes of large model pretraining in NLP and CV 
we leverage Equivariant Transformers (Section~\ref{sec:transformer}), which is a deep Transformer based model that can model complex interactions between atoms. Moreover, we propose a new training paradigm  (Section~\ref{sec:paradigm}) to make the model scale to multiple molecule training. We empirically show new SOTA performance in our \ourdata ~dataset, showing better generalization and simulation accuracy. 

\subsection{Force-centric Multi-molecule Optimization}

We optimize the following objective: 
\begin{equation}
    \expt_{x, \mathbf{r}_0} \left[\expt_{\mathbf{r}\sim \mathbb{T}^{\DFT}(x, \mathbf{r}_0, \thermo)}\left[ \left\Vert - \nabla\Phi_\theta(\mathbf{r}, \mathbf{z}) - F(\mathbf{r}, \mathbf{z}) \right\Vert^2_2 \right] \right], 
    \label{eqn:multi_mole_obj}
\end{equation}
where the differences between the forces prediction \(-\nabla \Phi_\theta (\mathbf{r}, \mathbf{z})\) and the ground-truth forces \(F(\mathbf{r},\mathbf{z})\) are minimized. The loss is optimized across multiple DFT trajectories on different types of polymers. 

\hide{
where we note two major differences: 
\begin{itemize}
    \item Firstly, the optimization objective for the potential energy function is dropped. In Section~\ref{prelim} we have noted the difficulty of the joint training on both the potential energy and forces in multi-molecule settings. To solve this, we train only on forces, which are local quantities defined on atoms and are more generalizable across different molecules. 
Empirically, forces are statistically of the same distribution in molecules, while energy distributions vary greatly, even after normalized by the number of atoms. 
    \item In addition to training on forces, our objective takes into account of the distributional variations in different trajectories of the same distribution. And because of our objective is compatible of multi-molecule training, we can train on various molecule families with different sizes, 
allowing the model to learn from more possibilities of atomic interactions and how they change according to the molecule size.
\end{itemize}
}


We justify our training objective for developing a machine learning forcefield for polymers. Our objective drops the optimization of the potential energy function and focuses solely on the forces.
As demonstrated in Section~\ref{prelim}, joint training on both potential energy and forces in multi-molecule settings is challenging.

Empirically, forces are local attributes defined on atoms and are statistically of the same distribution across different polymers. However, due to the complex quantum mechanical process, the distributions of the potential energy, which is a molecular-level attribute, vary greatly even after normalization. As a result, it is challenging for neural networks to accurately compute potential energy for multiple molecules without additional prior knowledge about the underlying quantum mechanics.
Therefore, training only on forces allows our model to be more generalizable across multiple molecules.

%due to the quantum mechanical process that vary 
Moreover, our objective takes into account the distributional variations in different trajectories of the same distribution, making it compatible with multi-molecule training. This allows our model to be trained on various molecule families with different sizes, providing the model with the opportunity to learn from more possibilities of atomic interactions and how they change according to the molecule size. By training on different molecules, our model can better generalize to unseen molecules, leading to more robust simulations.

\subsection{Energy Prediction}
Objective function~\eqref{eqn:multi_mole_obj} provides a supervision signal to the model only on the forces. However, the potential energy of the molecule during simulation is also an important indicator of the state of the molecule, for example, if the molecular conformation is in an equilibration state with energy fluctuating around a local minimum of the energy surface. 
In order to predict the potential energy for molecules during simulation, we note that by training exclusively on forces with~\eqref{eqn:multi_mole_obj}, the model output \(\Phi_\theta\) is linearly correlated with the ground-truth potential energy \(E\) (Figure~\ref{fig:model:energy_prediction}).  
We thus call \(\Phi_\theta\) \emph{pseudo-potential energy}. 
In order to predict \(E\) from \(\Phi_\theta\),
we can estimate \(E_t\) with \({E}_t=E_0 + \int_0^t \frac{\partial \Phi_\theta}{\partial \mathbf{r}}(\mathbf{r}_s, \mathbf{z})ds\) for a fixed time window \(t\in [0, T]\), where \(E_0\) is the initial energy of at the start of the simulation. The integral can be approximated with 
numeric Taylor expansion: 
\[
\overline{E}_t = \overline{E}_{t-1} - \left\langle \frac{\partial{\Phi}}{\partial{\mathbf{r}}}  (\mathbf{r}_{t-1}), \mathbf{r}_t - \mathbf{r}_{t-1} \right\rangle.
\]
Then given uniformly sampled \(0=t_0<\ldots<t_{m}=T\), we can estimate the potential energy function with 
\begin{eqnarray}
 & E^*(\mathbf{r}, \mathbf{z}) & =  \mathbf{W}_E \Phi_\theta(\mathbf{r}, \mathbf{z}) + \mathbf{b}_E, \nonumber \\
     \mathrm{where}\  & (\mathbf{W}_E, \mathbf{b}_E) & =  \arg\min \sum_{i=0}^m \Vert (\mathbf{W}_E \Phi_\theta + \mathbf{b}_E) - \overline{E}_i\Vert.
\end{eqnarray}

%An illustration of the energy prediction scheme is shown in Figure~\rui{put a figure here} \rui{and show the error vs numeric integration. }

%Mainstream machine learning forcefield optimize their parameters to find the minimum of 


\subsection{Comparison with Existing Methods}

 Existing graph neural network forcefields TorchMDNet~\citep{tholke2022torchmd}, SchNet~\citep{schutt2018schnet}, and GemNet~\citep{gasteiger2021gemnet} learn potential energy and forces from an MD trajectory of a single molecule from the MD17~\cite{chmiela2017machine} dataset. These models parameterize the potential energy as \(\Phi_\theta\) and forces as \(\frac{\partial \Phi_\theta}{\partial \mathbf{r}}\). 
 The joint optimization problem cannot na\"ively scale to multiple molecules, as shown in Table~\ref{table:demo_joint} and Figure~\ref{fig:single_multi_compare}.  \zc{??} While their methods perform well in predicting energy and forces on given trajectories, they cannot generalize well to multiple molecule training when multiple polymers are involved. Furthermore, their training and evaluation do not consider the robustness of MD simulations~\cite{fu2022forces}.

%They parameterized the energy function as $\Phi_\theta(\mathbf{r}, \mathbf{z})$, where $\theta$ is the parameter to be learned. The parameterized forces can be obtained through differentiation $\frac{\partial \Phi_\theta(\mathbf{r}, \mathbf{z})}{\partial \mathbf{r}}$.
\hide{
\begin{equation}
    \mathbf{E}_{\mathbf{r}\sim \mathbb{T}(x, \mathbf{r}_0, \thermo)}\left[ \Vert \Phi_\theta(\mathbf{r}, \mathbf{z}) - E(\mathbf{r}, \mathbf{z}) \Vert + \left\Vert \frac{\partial \Phi_\theta(\mathbf{r}, \mathbf{z})}{\partial \mathbf{r}} - F(\mathbf{r}, \mathbf{z}) \right\Vert \right],
    \label{eqn:single_mol_obj}
\end{equation}
\begin{equation}
    \mathbf{E}_{\mathbf{r}\sim \mathbb{T}(x, \mathbf{r}_0, \thermo)}\left[ \Vert \Phi_\theta(\mathbf{r}, \mathbf{z}) - E(\mathbf{r}, \mathbf{z}) \Vert + \left\Vert \frac{\partial \Phi_\theta(\mathbf{r}, \mathbf{z})}{\partial \mathbf{r}} - F(\mathbf{r}, \mathbf{z}) \right\Vert \right],
    \label{eqn:single_mol_obj}
\end{equation}

where \( \Phi_\theta(\mathbf{r}, \mathbf{z}) =\sum_i \Phi^i_\theta(\mathbf{r}, \mathbf{z})\), with each component in the sum being the hypothetical atomistic potential energy function. 
There are several mismatches between this objective and a multi-molecule model for simulations. Firstly, the potential energy function is formed as the simple sum of atomistic potential energy, which is an oversimplification of the real quantum mechanics at work. The lack of atomic-level information on potential energy makes it hard to train the model generalizable to multiple molecules. Secondly, as shown in Section~\ref{prelim}, the joint optimization of energy and forces is problematic in multi-molecule settings, leading to a deterioration of accuracy. Finally, the model is trained on a limited data region generated by a single MD simulation setting. As shown in Section~\ref{prelim}, the model performing well in this objective does not necessarily work in a realistic MD simulation. }

The sGDML model, as described in \cite{chmiela2017machine,chmiela2018towards}, directly outputs forces but not energy. sGDML is a small-scale kernel-regression-based algorithm that requires solving a normal equation that scales quadratically with the model parameter space, which prevents their model capacity to scale up or extend to multiple-molecule settings. \ours~could utilize the high model capacity of deep learning models to scale up performance with more multi-molecule data.  Additionally, \ours~ has the added benefit of allowing the model to output a \emph{pseudo-potential}, that is linearly correlated with the ground-truth potential energy. In simulations, sGDML relies on numeric integration to obtain potential energies along the trajectory, which can lead to error propagation. In contrast, our pseudo-potential provides an estimate of the ground-truth energy with a fixed error distribution that remains stable throughout the simulation.

%There are two main obstacles in this objective. Firstly, the joint optimization of energy and forces is difficult and even untrainable, especially when multiple molecules are concerned, as we have demonstrated in Section~\ref{prelim:gen}. This makes the trained model unstable in simulation and hard to scale to multi-molecule settings, and making generalization to unseen molecules infeasible. Furthermore, the model parameters are optimized on a single fixed trajectory of a single molecule, undermining the model's robustness in real simulations. 

%Classical forcefield bypass these problems by using physiochemistrical functionals that approximate the potential energy surface with prior physical knowledge. While with such knowledge can help learning the energy and forces with certain classes of molecular structures, no general approximation form could exist for arbitrary molecular structures. We therefore do not limit our model to fit certain approximation form of the potential energy, but instead utilize the rich representation ability of deep Equivariant Transformers to learn more universal forcefields. 


==> prelim.tex <==
\section{{Problem and Challenges}}
\label{prelim}





%We first investigate the difficulties of deploying existing state-of-the-art machine learning forcefields for polymers. While machine learning has demonstrated high accuracy and efficiency in small molecules and proteins in tasks such as property prediction and conformation generation, there is no feasible solution to apply them to polymers due to the lack of generalization ability and robustness in simulations. 

%The first difficulty in generalization ability is investigated in Section~\ref{prelim:gen}. Existing literature focuses extensively on training a separate model for different molecules for potential energy and forces prediction. We demonstrate that na\"ively extending their work to include multiple molecules could lead to deterioration in performance. The second difficulty is that even if a model is well trained for a single molecule, we show in Section~\ref{prelim:sim} that such models would not perform well in simulations. 
\paragraph*{Problem Definition.}
We represent a molecule as \(x\). Assuming \(n_x\) is the number of atoms, we represent the distribution of its conformations as \(\mathbf{r}_x\in \RR^{n_x\times 3}\) and the atom types of the molecule as \(\mathbf{z}_x\in \RR^{n_x}\). The potential energy of a molecule is determined given the conformation \(\mathbf{r}\sim\mathbf{r}_x\) and atom types, denoted as \(E=E(\mathbf{r}, \mathbf{z})\in\RR\). The forces applied on the atoms are obtained by \(F=-\frac{\partial E}{\partial \mathbf{r}}\in\RR^{n_x\times 3}\). In theory, a stable conformation is one where the potential energy achieves local minimum with zero forces. In MD simulations, the molecular conformations are moved according to forces and the thermostat of the simulation. We can denote the distribution of the conformation in a DFT-based MD simulation given a certain thermostat \(\thermo\) as 
\(\mathbb{T}^{\DFT}(x, \mathbf{r}_0, \thermo)\). We would omit the boundary conditions \((x, \mathbf{r}_0, \thermo)\) unless necessary. 
%Because of the energy injection in the simulation, the conformations from this distribution are likely equipped with non-zero forces. 


In this paper we use DFT potential energy and forces as references. Machine learning forcefields learn a model \(\Phi_\theta\) parameterized by \(\theta\) that approximates the DFT potential energy and forces: \(\Phi_\theta:(\mathbf{r},\mathbf{z}) \rightarrow (E^{\DFT}, F^{\DFT})\). 

The desired parameterization of \(\Phi\) should satisfy
\begin{equation}
    \theta = \arg\min \expt^{\ML}\left[ \Vert E^{\ML} - E^{\DFT}\Vert^2_2 + \Vert F^{\ML} - F^{\DFT}\Vert^2_2 \right] \nonumber
\end{equation}
where \(\expt^{\ML}\) samples conformation from \(\mathbb{T}^{\ML}\), representing the MD trajectories generated by \(\Phi_\theta\). However, this formula is intractable to optimize since the expectation depends on the model itself. Instead, in practice, the expectation is taken w.r.t. DFT trajectory:
\begin{equation}
    \theta = \arg\min \expt^{\DFT}\left[ \Vert E^{\ML} - E^{\DFT}\Vert^2_2 + \Vert F^{\ML} - F^{\DFT}\Vert^2_2 \right] \label{eqn:mainstream_optim}
\end{equation}

\paragraph*{However, this formulation has been observed to suffer from simulation instability~\cite{fu2022forces}, as it does not necessarily guarantee the accuracy of \(\Phi_\theta\) in its own trajectory. } In most machine learning forcefield literature, the forcefield performance is only reported on DFT trajectories. \citet{fu2022forces} analyzed the state-of-the-art machine learning forcefields in simulation and reported that they are not necessarily accurate when generating their own trajectoreis, leading to instable simulations and worsened downstream task performance. In Table~\ref{tab:sim_robustness_6loop} we experimented with the state-of-the-art methods in simulation scenarios and found that their trajectoreis would ``collapse'' after a short period of time, indicating that a forces error on \(\mathbb{T}^{\DFT}\) does not imply the same on \(\mathbb{T}^{\ML}\). 

\paragraph*{Furthermore, such formulation cannot na\"ively extend to training on multiple molecules.} \hide{Here we demonstrate a simple experiment where we consider the cycloalkane family from cyclopropane to cycloheptane, which are similar ring structures consisting of 3 to 7 methylene groups. The molecular formula for them is \((\mathrm{CH}_2)_3\), \((\mathrm{CH}_2)_4\), \(\ldots\), \((\mathrm{CH}_2)_7\). We consider three different state-of-the-art equivariant graph neural networks: TorchMDNet~\cite{tholke2022torchmd}, GemNet~\cite{gasteiger2021gemnet}, and NequIP~\cite{batzner20223}. For each model, we train jointly on the 5 molecules, with \(10,000\) data for training, \(1,000\) for validation, and \(5,000\) for testing for each of the molecules. 

In Table~\ref{table:demo_joint}, we report the \emph{Mean Absolute Error} (MAE) of ML forces compared to DFT forces on the three models, averaged across all 5 molecules. Comparison is made between the models trained and evaluated separately on different molecules - Separate, and a unified model trained and evaluated simultaneously on 5 molecules - Joint. 
Notably, across all three models, more data from different molecules does not improve the performance. Instead, they make the model perform two to three times worse than separately trained models. 

\input{tables/demo_naive_multimodel.tex}
}

In Figure~\ref{fig:prelim:optim} we display the validation loss of the energy and forces in training. ``Original'' means the mainstream single-molecule training paradigm, and ``\ours'' represents our improved training paradigm. During training, our paradigm achieves an order of magnitude lower validation loss and stabler loss curve, whereas the forces validation loss is particularly volatile for the original training paradigm. To explain why this phenomenon occurs,
we analyze the distributions of the per-atom potential energy and the distributions of forces in Figure~\ref{fig:prelim:dist}. The forces share a similar distribution for all polymers. The per-atom potential energy distribution for each polymer varies greatly, which depends on not only the system size but also the type of polymer. The potential energy distribution as a whole is also a very different distribution than the forces. 
This reveals that the optimization of the potential energy and forces could be at conflict, resulting in volatility in training and decreased performance. 


\begin{figure}[tp]
    \centering
    \subfigure[Optimization Curves.]{\includegraphics[width=0.9\linewidth]{figs/validation_loss_curve.pdf}\label{fig:prelim:optim}}

    \subfigure[Energy and Forces Distributions.]{\includegraphics[width=0.9\linewidth]{figs/energy_forces_dist.pdf}\label{fig:prelim:dist}}
    \caption{Illustration of the optimization bottleneck in the existing deep learning forcefield training paradigm. Figure~\ref{fig:prelim:optim} shows the validation loss curve of Equivariant Transformers in the original training paradigm and in the PolyGET training paradigm. With the original paradigm, both the energy and forces are unstable and result in less generalizable models. Figure~\ref{fig:prelim:dist} shows the distribution of per-atom potential energies and forces across different polymers. It can be observed that forces follow the same distribution for different types of polymers, while the per-atom potential energy does not. We assume the mismatch between the potential energy and forces distributions is the cause of the optimization bottleneck. }
    \label{fig:prelim}
\end{figure}






%We address these challenges in the following section. 
% \zc{ It feels strange to have a hanging sentence as a single paragraph. either expand it, or remove it.} 


\hide{

\subsection{Simulation Robustness}
\label{prelim:sim}

Although machine learning models for force field prediction have shown state-of-the-art performance, their training and evaluation are often based on the static evaluation of molecule conformations using a DFT trajectory. However, this approach does not necessarily reflect the performance of these models in a dynamic MD simulation, where the model is expected to predict forces for a trajectory of conformations. In a static evaluation setting, the model predicts forces for a single conformation that is reliably simulated by DFT forces. In contrast, in an MD simulation, the model is expected to produce a trajectory of predicted forces.

Empirical evidence from \citet{fu2022forces} and Table~\ref{tab:sim_robustness_6loop} has shown that good model performance on a single trajectory does not guarantee that the model can produce a reliable simulation trajectory on its own. This is because one trajectory only covers limited types of quantum mechanical interactions between atoms, and models trained and evaluated in such ways may not perform well in unknown scenarios where noises are introduced in MD simulations. Therefore, it is crucial to test the robustness of these models by evaluating their performance on a variety of MD simulations that include different types of interactions and environments.

\subsection{Key Solution: Equivariant Transformer-based Forcefield for Multiple Molecule Training}

 \zc{ This can be moved to your  method  section.} 
To solve the two problems, the key solution is to scale the model to parameterize forcefields for multiple molecules. If this is achieved, then the model will be hoping to a) implicitly learn the transferable quantum mechanics underlying different molecules, leading to better generalization ability; and b) handle the more diverse conformations in simulation environments, as the model has seen more types of quantum interactions between atoms. 
To be able to achieve these, the model will need to have strong representation ability. 
Inspired by recent successes of large model pretraining in NLP and CV \rui{cite? } 
we leverage Equivariant Transformers (Section~\ref{sec:transformer}), which is a deep Transformer based model that can model complex interactions between atoms. Moreover, we propose a new training paradigm  (Section~\ref{sec:paradigm}) to make the model scale to multiple molecule training. We empirically show new SOTA performance in our \ourdata dataset, showing better generalization (Section~\ref{sec:exp:multimolecule}), and MD simulations (Section~\ref{sec:exp:sim}). 
}


==> short_versions/prelim.tex <==
\section{Problem and Challenges}
\label{prelim}
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/sota_robustness.pdf}
    \caption{State-of-the-art machine learning forcefields fail critically in polymer simulations. We take the 6-loop polymerization of 3 example polymer families (Table~\ref{table:data} and run  }
    \label{fig:sim_robustness_6loop}
\end{figure}

\hide{

\newcommand{\finished}[1]{\(\rm{#1}\)}
\newcommand{\unfinished}[1]{\(\rm{#1}^*\)}
\begin{table}[]
\begin{tabular}{llll}
Polymer & Method     & Steps @ 1-loop & Steps @ 6-loop \\
CK6     & NequIP     & 123K           & 50K            \\
        & TorchMDNet & 238K           & 65K            \\
        & \ours       & \unfinished{600K}           & \unfinished{600K}           \\ \hline
LAC8    & NequIP     & 82K            & 43K            \\
        & TorchMDNet & 143K           & 83K            \\
        & \ours       & \unfinished{600K}           & \unfinished{600K}          \\ \hline
ETH     & NequIP     & 50K            & 38K            \\
        & TorchMDNet & 78K            & 54K            \\
        & \ours       & \unfinished{600K}           & \unfinished{600K}           \\ \hline
OTH8    & NequIP     & 8K             & 6K             \\
        & TorchMDNet & 16K            & 12K            \\
        & \ours       & \unfinished{600K}           & \unfinished{600K}         
\end{tabular}
\caption{Simulation Robustness. For each example polymer we run simulations with baseline forcefield and \ours~ for a maximum of 600K steps to test the robustness of each forcefield in the simulation. \unfinished{600K} means that the simulation kept running after 600K steps. \rui{figure instead}}
\label{tab:sim_robustness_6loop}
\end{table}
}



\paragraph*{Challenges. } This formulation has been observed to suffer from simulation instability and struggles with training on multiple molecules. 
%In Table~\ref{tab:sim_robustness_6loop}, we measure how far can state-of-the-art machine learning forcefields can run MD simulations without collapsing. We define the collapsing of an MD simulation by the point where the simulated polymer  we found that state-of-the-art methods' trajectories would collapse after a short period, indicating that force error on  \(\mathbb{T}^{\DFT}\) does not imply the same on \(\mathbf{T}^{\ML}\). 


We note that the evaluation of existing deep learning forcefields focuses prevalently on comparing the predicted forces with the reference data on given golden MD trajectories. However, this does not translate to good performance when the forcefield is tasked to run its own simulation. 
In Figure~\ref{fig:sim_robustness_6loop}, we visualize example MD simulations with TorchMD-Net~\cite{tholke2022torchmd}, one of the most accurate deep learning models for molecular forces prediction. The figures show that after running for a short period of time, the model could not maintain high accuracy, eventually leading to the polymer structure breaking apart. A similar phenomenon is noted by \citet{fu2022forces}. This is not ideal when MD simulations are required to study the ensemble properties of polymers. 

Furthermore, existing ML forcefields focus on training separate models for different molecules~\cite{tholke2022torchmd,schutt2018schnet,batzner20223,fuchs2020se}. We find that the extension to multi-molecule training, i.e. training a unified ML forcefield for different types of molecules is not straightforward. 
In Figure~\ref{fig:prelim:optim}, we display the validation loss of the energy and forces in training. Our improved training paradigm, ``\ours'', achieves lower validation loss and a more stable loss curve than the mainstream single-molecule training paradigm, ``Original''. The optimization bottleneck in the existing deep learning forcefield training paradigm can be explained by analyzing the per-atom potential energy and force distributions in Figure~\ref{fig:prelim:dist}. This reveals that the optimization of the potential energy and forces could be in conflict, resulting in volatility in training and decreased performance.

\paragraph*{Challenges. } State-of-the-art EGNN models built upon this learning objective suffer from two key challenges: (1)
they struggles with learning from  multiple molecules; and (2) they suffer from 
simulation instability although they can achieve high accuracy in static force prediction.
In Figure~\ref{fig:prelim:optim},
 we show that when training one unified model for multiple molecules, the performance of existing EGNN models decrease rather than increase.
 \zc{ I don't really agree with Rempy that this section can be cut.  The corresponding content can be moved to introduction section, method section, and experiment section.} 


 The optimization bottleneck in the existing deep learning forcefield training paradigm can be explained by analyzing the per-atom potential energy and force distributions in Figure~\ref{fig:prelim:dist}. This reveals that the optimization of the potential energy and forces could be at conflict, resulting in volatility in training and decreased performance.
 \zc{ This is better to be put into the method section.} 


\begin{figure}[h]
    \centering
    \subfigure[Optimization Curves.]{\includegraphics[width=0.9\linewidth]{figs/validation_loss_curve.pdf}\label{fig:prelim:optim}}

    \subfigure[Energy and Forces Distributions.]{\includegraphics[width=0.9\linewidth]{figs/energy_forces_dist.pdf}\label{fig:prelim:dist}}
    \caption{Illustration of the optimization bottleneck in the existing deep learning forcefield training paradigm. Figure~\ref{fig:prelim:optim} shows the validation loss curve of Equivariant Transformers in the original training paradigm and in the PolyGET training paradigm. With the original paradigm, both the energy and forces are unstable and result in less generalizable models. Figure~\ref{fig:prelim:dist} shows the distribution of per-atom potential energies and forces across different polymers. It can be observed that forces follow the same distribution for different types of polymers, while the per-atom potential energy does not. We assume the mismatch between the potential energy and forces distributions is the cause of the optimization bottleneck.  \zc{  The first first figure can be moved to the experiment to show that our measure can harness multi-molecule training. The second subfigure should be moved into the method  section to motivate why we just train over force.} }
    \label{fig:prelim}
\end{figure}



In Table~\ref{tab:sim_robustness_6loop}, we measure how far can state-of-the-art machine learning forcefields can run MD simulations without collapsing. We define the collapsing of an MD simulation by the point where the simulated polymer  we found that state-of-the-art methods' trajectories would collapse after a short period, indicating that force error on  \(\mathbb{T}^{\DFT}\) does not imply the same on \(\mathbf{T}^{\ML}\). 
 \zc{ This is better to be presented in the experiment section.} 


==> tables/demo_naive_multimodel.tex <==


\hide{\begin{table}[h]
    \begin{tabular}{lllll}
               &   Training     & MAE (eV/A) & Max.  & Std.  \\
    \multirow{2}{*}{GemNet} & Joint &  0.088      & 0.741 & 0.054 \\
     & Separate & 0.037      & 0.119 & 0.021 \\ \hline
     \multirow{2}{*}{NequIP} & Joint &   0.075      & 0.732 & 0.051 \\
     & Separate &  0.034      & 0.115 & 0.018 \\ \hline
    \multirow{2}{*}{TorchMDNet} & Joint      & 0.062      & 0.618 & 0.040 \\
     & Separate     & 0.025      & 0.092 & 0.016 \\ \hline
    \end{tabular}
    \caption{Demonstration of na\"ive multi-molecule training on SOTA GNN forcefields. \emph{Joint} means the model is trained and evaluated on all monomers simultaneously with a single model. \emph{Separate} means different models are trained and evaluated on a single molecule system separately, and results are averaged across all monomers. }
    \label{table:demo_joint}
\end{table}}


==> tables/monomer_eval.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
        \textbf{Polymer} & \multicolumn{2}{c}{\textbf{NequIP}} & \multicolumn{2}{c}{\textbf{TorchMDNet}}  & \multicolumn{2}{c}{\textbf{SchNet}} & \multicolumn{2}{c}{\textbf{DEPT}} \\ \hline
        \textbf{} & MAE & CosD & MAE & CosD & MAE & CosD & MAE & CosD \\ 
        \textbf{994} & 0.065 & 8.6625 & 0.027 & 3.0844 & 0.362 & 177.6066 & 0.006 & 0.0914 \\ 
        \textbf{51} & 0.099 & 18.6465 & 0.022 & 0.8516 & 0.246 & 120.5511 & 0.007 & 0.1076 \\ 
        \textbf{53} & 0.070 & 7.6316 & 0.016 & 0.3211 & 0.299 & 135.5392 & 0.004 & 0.0245 \\ 
        \textbf{993} & 0.067 & 8.5264 & 0.028 & 1.4672 & 0.387 & 165.0499 & 0.007 & 0.0885 \\ 
        \textbf{49} & 0.091 & 11.4420 & 0.022 & 0.6439 & 0.236 & 82.1604 & 0.005 & 0.0307 \\ 
        \textbf{1054} & 0.089 & 15.6643 & 0.070 & 13.2913 & 0.710 & 350.9559 & 0.010 & 0.1551 \\ 
        \textbf{1058} & 0.075 & 9.0184 & 0.097 & 14.5652 & 0.783 & 475.4124 & 0.007 & 0.0858 \\ 
        \textbf{1060} & 0.109 & 12.2400 & 0.028 & 0.8014 & 0.316 & 90.5123 & 0.007 & 0.0511 \\ 
        \textbf{1056} & 0.098 & 17.2831 & 0.082 & 9.4748 & 1.111 & 578.8684 & 0.009 & 0.1162 \\ 
        \textbf{5} & 0.096 & 17.0552 & 0.032 & 1.3555 & 0.320 & 130.9253 & 0.008 & 0.0924 \\ 
        \textbf{15} & 0.111 & 29.7486 & 0.024 & 0.9334 & 0.474 & 217.7669 & 0.007 & 0.1052 \\ 
        \textbf{7} & 0.099 & 13.1006 & 0.025 & 0.9263 & 0.308 & 111.0542 & 0.006 & 0.0384 \\ 
        \textbf{1052} & 0.083 & 8.7094 & 0.121 & 18.1693 & 1.097 & 427.8985 & 0.011 & 0.1251 \\ 
        \textbf{1053} & 0.082 & 12.8490 & 0.037 & 2.0404 & 0.415 & 170.1131 & 0.007 & 0.0800 \\ 
        \textbf{1055} & 0.069 & 7.1176 & 0.037 & 1.9163 & 0.487 & 239.7282 & 0.006 & 0.0453 \\ 
        \textbf{1} & 0.116 & 17.7811 & 0.037 & 1.6518 & 0.430 & 216.4268 & 0.008 & 0.0864 \\ 
        \textbf{9} & 0.084 & 14.3924 & 0.045 & 3.0562 & 0.634 & 346.0937 & 0.008 & 0.1131 \\ 
        \textbf{3} & 0.091 & 16.0852 & 0.046 & 3.4579 & 0.512 & 257.3273 & 0.009 & 0.1215 \\ 
        \textbf{1050} & 0.114 & 22.3451 & 0.055 & 5.9015 & 0.334 & 151.6124 & 0.011 & 0.1790 \\ 
        \textbf{50} & 0.132 & 30.1971 & 0.030 & 1.0716 & 0.366 & 164.2241 & 0.006 & 0.0439 \\ 
        \textbf{52} & 0.123 & 41.3205 & 0.023 & 0.7411 & 0.345 & 111.5990 & 0.008 & 0.0679 \\ 
        \textbf{11} & 0.086 & 11.4972 & 0.042 & 2.2244 & 0.515 & 240.8465 & 0.008 & 0.1033 \\ 
        \textbf{17} & 0.073 & 8.1809 & 0.022 & 0.5612 & 0.347 & 110.0944 & 0.006 & 0.0421 \\ 
    \end{tabular}
    \caption{Multi-molecule monomer}
\end{table*}
